Model-Targeted Poisoning Attacks with Provable Convergence

In a poisoning attack, an adversary with control over a small fraction of the training data attempts to select that data in a way that induces a corrupted model that misbehaves in favor of the adversary. We consider poisoning attacks against convex machine learning models and propose an efficient poisoning attack designed to induce a specified model. Unlike previous model-targeted poisoning attacks, our attack comes with provable convergence to {\it any} attainable target classifier. The distance from the induced classifier to the target classifier is inversely proportional to the square root of the number of poisoning points. We also provide a lower bound on the minimum number of poisoning points needed to achieve a given target classifier. Our method uses online convex optimization, so finds poisoning points incrementally. This provides more flexibility than previous attacks which require a priori assumption about the number of poisoning points. Our attack is the first model-targeted poisoning attack that provides provable convergence for convex models, and in our experiments, it either exceeds or matches state-of-the-art attacks in terms of attack success rate and distance to the target model.

==> experiments_copy.tex <==
\section{Experiments}
\label{sec:experiments}

We first describe our experimental setup regarding the datasets, models, attacks and target classifiers. Next, we present the experimental results by showing the convergence of Algorithm~\ref{algorithm}, the comparison of attack success rates to state-of-the-art poisoning attack, and the theoretical lower bound for inducing a given target classifier and its gap to the number of poisoning points used by our attack. 
%All of our evaluatuion code is available at: \url{https://github.com/suyeecav/model-targeted-poisoning}.

We experiment on both the (practical) subpopulation on the and the conventional indiscriminate attack scenarios. Due to space limitation, in the main body of the paper, we only include the results of SVM model on the Adult~\citep{Dua:2019} and the Dogfish datasets~\citep{koh2017understanding}. Results of SVM model on the \MNIST dataset and logistic regression model on the three datasets are deferred to the Appendix. 

We are most interested in subpopulation attacks, since they correspond to the more realistic attacker goal of impacting the classifier outputs for a targeted subpopulation. Therefore, in the main body, we introduce the results of SVM model on the Adult dataset~\citep{Dua:2019} in the subpopulation poisoning scenario. For completeness, we also evaluate our attack on SVM model on \MNIST\ dataset in the indiscriminate poisoning scenario but defer details on those experiments to Appendix~\ref{sec:indiscriminate_attack}. Our findings for the indiscriminate attacks are that the attack gradually and consistently converges to the target model in terms of the maximum loss difference and the Euclidean distance to the target, with attack success rates that are comparable to the state-of-the-art attack (unlike the subpopulation attacks, where our attack produces superior results). To further verify the universal effectiveness of our attack, we also evaluate our attack on additional dataset (Dogfish) and model (logistic regression), and more details can be found in Appendix~\ref{sec:additional_exps}.
%and 2) our attack has comparable attack success rates with the SOTA poisoning attack, and 3) there exists relatively large gap between the lower bound and the number of poisoned points of models generated from our attack and the SOTA poisoning attack. Next, we provide more details regarding the subpopulation attack scenario.

\shortsection{Dataset, Model and Attacks} For the subpopulation attack experiments, we use the Adult dataset~\citep{Dua:2019}. This dataset was used for evaluation by the first subpopulation attack paper~\citep{jagielski2019subpop}.
We downsampled the Adult dataset to ensure it is class-balanced and we ended up having 15,682 training and 7,692 test examples.
We conduct experiments on linear SVM model and compare our model-targeted poisoning attack in Algorithm~\ref{algorithm} to the state-of-the-art KKT attack~\citep{koh2018stronger}. We do not include the model-targeted attack from~\citet{mei2015using} because it underperforms the KKT attack~\citep{koh2018stronger}. We also do not include objective-driven attacks because our main goal here is to evaluate how well our attack approaches a given target model, across a range of target models. Model-targeted attacks can be compared to objective-driven attacks with regards to a given attacker objective by choosing the target model in a careful way. We show some heuristics of choosing such target models and show that, when the target models are carefully selected, our attack can also outperform the state-of-the-art objective-driven attack in Appendix~\ref{sec:model_vs_objective}. 

%We do not include the two other strong attacks in our evaluation. We exclude the influence attack~\citep{koh2017understanding,koh2018stronger} because it slightly underperforms the KKT attack, does not work with a target classifier, and is also slow. We exclude the min-max attack~\citep{steinhardt2017certified,koh2018stronger} because it only works for the indiscriminate scenario and does not use a target classifier in the attack process. The simple random label-flipping attack for subpopulation~\citep{jagielski2019subpop} is not considered either because it consistently underperforms the KKT attack.

Both our attack and the KKT attack take as input a target classifier and the original training data, and output a set of poisoning points selected with the goal that the induced classifier is as close as possible to the target classifier. We compare the effectiveness of the attacks in selecting poisoning points that converge to a given target classifier by testing the attacks using the same target model.

The KKT attack requires a target number of poisoning points as an input while our attack is more flexible and can either take a target number of poisoning points or a threshold for $\epsilon$-close distance to the target model. Since we do not know the number of poisoning points needed to reach some attacker goal in advance for the KKT attack, we first run our attack and produce a classifier that satisfies the selected $\epsilon$-close distance threshold. The loss function is set as the hinge loss since we target an SVM model in our experiments and we set $\epsilon = 0.01$ for all these experiments. Then, we use the size of the poisoning set returned from our attack (denoted by $n_p$) as the input to the KKT attack for the target number of poisons needed. We also compare the two attacks with varying numbers of poisoning points up to $n_p$. 
For the KKT attack, its entire optimization process must be rerun
whenever the target number of poisoning points changes. Hence, it is infeasible to evaluate the KKT attack on many different poisoning set sizes. In our experiments, we run the KKT attack five poisoning set sizes: $0.2 \cdot n_p$, $0.4 \cdot n_p$, $0.6 \cdot n_p$, $0.8 \cdot n_p$, and $n_p$. In contrast, we simply run our attack for iterations up to the maximum number of poisoning points, collecting a data point for iteration up to $n_p$. 


\shortsection{Subpopulations} We identify the subpopulations for the Adult dataset using $k$-means clustering techniques (ClusterMatch~\citep{jagielski2019subpop}) to obtain different clusters ($k=20$ in our case). For each cluster, we select instances with label ``<=50K'' to form the subpopulation (indicating all instances in the subpopulation are in low income group). This way of defining subpopulation is rather arbitrary (in constrast to a more likely attack goal which would select subpopulations based on demographic characteristics), but enables us to simplify the analysis. From the $20$ subpopulations obtained, we select three subpopulations with the highest test accuracy on the clean model and they all have 100\% test accuracy, indicating all instances in these subpopulations are correctly classified as low income. This enables us to use ``attack success rate'' and ``accuracy'' without any ambiguity on the subpopulation---for each of our subpopulations, all instances are originally classified as low income, and the simulated attacker's goal is to have them classified as high income. 
%Size of the subpopulations (Cluster 0-2) are XX, XX and XX respectively. 

For each subpopulation, we use the heuristic approach from~\citet{koh2018stronger} to generate a target classifier that has 0\% accuracy (100\% attacker success) on the subpopulation, indicating that all subpopulation instances are now classified as high income. 
%\shortsection{Subpopulation and Target Classifier} For the Adult dataset, the subpopulations are identified first using the $k$-means clustering techniques to obtain different clusters ($k=20$ in our case) (ClusterMatch~\citep{jagielski2019subpop}) and for each cluster, we only select instances with label ``<=50K'' and form the subpopulation (indicating all instances in the subpopulation are in low income group). This way of defining subpopulation is rather arbitrary, but enables us to simplify the analysis and we can also use the ``attack success rate'' and ``accuracy'' without any ambiguity on the subpopulation. From the $20$ subpopulations obtained, we select three subpopulations with the highest test accuracy on the clean model and all the three ended up having 100\% test accuracy on subpopulation, indicating all instances are correctly classified into low income group. For each subpopulation, we generate a target classifier that has 0\% accuracy on the subpopulation, indicating all subpopulation instances are now in high income group. To generate the target classifier that satisfies the goal, we adopt the heuristic approach from~\citet{koh2018stronger}.
%, but in contrast to the indiscriminate setting, here we only select high loss training points from the subpopulation in the training set.

%More details regarding the datasets can be found in 
%MNIST-17 consists of 13,007 training examples and 2,163 test examples, and is commonly used in evaluating the conventional poisoning attack.  We downsample the Adult data and perform one-hot encoding for the discrete features, and end up with a dataset of 57 features, 15,682 training data and 7,692 test data. Features of both datasets are normalized by their maximum value per feature and the processed features all lie in range $[0,1]$ (except for binary features of Adult dataset). We conduct experiments on linear SVM models and we set the regularization constant $C_R = 0.09$ for both datasets. 

    \begin{figure}[tb]
        \centering
        \begin{subfigure}[b]{0.4\textwidth} 
            \centering 
            \includegraphics[width=0.9\textwidth]{figures/adult/svm/subpop-0_max_loss_diff_tol-0.01_err-1.0.png}
            \caption[]%
            {Max Loss Difference}    
            \label{fig:adult_svm_subpop0_max_loss_diff}
        \end{subfigure}
        \begin{subfigure}[b]{0.4\textwidth} 
            \centering 
        \includegraphics[width=0.9\textwidth]{figures/adult/svm/subpop-0_norm_diff_tol-0.01_err-1.0.png}
            \caption[]%
            {Euclidean Distance}    
            \label{fig:adult_svm_subpop0_norm_diff}
        \end{subfigure}
        \caption[]
        {Attack convergence (results shown are for the first subpopulation, Cluster 0). The maximum number of poisons is set using the $0.01$-close threshold to target classifier.}
        \label{fig:adult_svm_subpop0_convergence}
    \end{figure}

\shortsection{Convergence}
Figure~\ref{fig:adult_svm_subpop0_convergence} shows the convergence of Algorithm~\ref{algorithm} using both maximum loss difference and Euclidean distance to the target.  The maximum number of poisons ($n_p$) for the experiments is obtained when the classifier from Algorithm~\ref{algorithm} is $0.01$-close to the target classifier. Our attack steadily reduces the maximum loss difference and Euclidean distance to the target model, in contrast to the KKT attack which does not seem to converge towards the target model reliably. 
%\dnote{I don't understand the next sentence (2\% of what?) or how it fits with what I seen in the graphs:} 
Concretely, at the maximum number of poisons in Figure~\ref{fig:adult_svm_subpop0_convergence}, both the maximum loss difference and Euclidean distance of our attack (to the target) is less than 2\% of the corresponding distances of the KKT attack. 

%\dnote{If you can, please make graphs with larger fonts for all the labels, and with keys that are not overlapping, or nearly overlapping the data points. Ideally, they would also have a more horizontal aspect ratio (wider for the same height) to use the space better.}

\shortsection{Attack Success}
Next, we compare the classifiers induced by the two attacks in terms of the attacker's goal of reducing the test accuracy on the subpopulation. 
Figure~\ref{fig:adult_svm_subpop_acc} shows the accuracy results for the three subpopulations. For each test, the maximum number of poisoning points is obtained by running our attack with a target of $0.01$-closeness (in loss-based distance). For the three subpopulations, at the maximum number of poisons, our attack is much more successful than the KKT attack---the induced classifiers have 0.5\% accuracy compared to 15.4\% accuracy for KKT on subpopulation 1, 0.0\% compared to 6.9\% on subpoulation 2, and 0.3\% compared to 20.1\% on subpoplation 3. 


Our attack outperforms the KKT attack both in terms of the convergence and attack success. We suspect the main reason is related to how we approach the target classifier. The foundation of the KKT attack is that, for binary classification, any target classifier generated by training on set $D_c$ with size $n$, the (exact) same classifier can also be obtained by training on set $D'_c$ with size at most $n$ and this training set only contains two distinct points, one from each class. In practice, KKT attack often aims to induce the exact same classifier with much smaller number of poisoning points, which may not be feasible and then KKT attack fails in these situations. In contrast, our attack does not try to obtain the exact classifier and only tries to approach it with the minimum number of poisoning points. Therefore, often we can get close to the target classifier with fewer poisoning points than the number of points used to exactly produce the target classifier. However, this is not guaranteed and occasionally may not happen. For example, in the indiscriminate attack scenario on MNIST 1--7 dataset (Appendix~\ref{sec:additional_exps}), the KKT attack sometimes slightly outperforms our attack.


    \begin{figure*}[tb]
        \centering
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \includegraphics[width=0.9\textwidth]{figures/adult/svm/subpop-0_acc_score_tol-0.01_err-1.0.png}
            \caption[]{Cluster 0} 
            \label{fig:adult_svm_subpop0_acc_scores}
        \end{subfigure}
        \begin{subfigure}[b]{0.3\textwidth}  
            \centering 
            \includegraphics[width=0.9\textwidth]{figures/adult/svm/subpop-1_acc_score_tol-0.01_err-1.0.png}
            \caption[]{Cluster 1}    
            \label{fig:adult_svm_subpop1_acc_scores}
        \end{subfigure}
        \begin{subfigure}[b]{0.3\textwidth}  
            \centering 
            \includegraphics[width=0.9\textwidth]{figures/adult/svm/subpop-2_acc_score_tol-0.01_err-1.0.png}
            \caption[]{Cluster 2}    
            \label{fig:adult_svm_subpop2_acc_scores}
        \end{subfigure}
        \caption[]{Test accuracy for each subpopulation with classifiers induced by poisoning points obtained from our attack and the KKT attack.} 
        \label{fig:adult_svm_subpop_acc}
    \end{figure*}

    \begin{figure*}[t]
        \centering
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            % \includegraphics[width=\textwidth]{imgs/metric_compare_degenerate/cifar10-madry/untargeted/diff_metrics_densenet_resnet_autozoom.png}
            \includegraphics[width=0.9\textwidth]{figures/dogfish/svm/whole-0_acc_score_tol-2.0_err-0.1.png}
           \caption[]
            {10\% Error Rate} 
            \label{fig:dogfish_svm_01_acc}
        \end{subfigure}
        %\hfill
        \begin{subfigure}[b]{0.3\textwidth} 
            \centering 
            \includegraphics[width=0.9\textwidth]{figures/dogfish/svm/whole-0_acc_score_tol-2.0_err-0.2.png}
            \caption[]%
            {20\% Error Rate}    
            \label{fig:dogfish_svm_02_acc}
        \end{subfigure}
        \begin{subfigure}[b]{0.3\textwidth} 
            \centering 
            \includegraphics[width=0.9\textwidth]{figures/dogfish/svm/whole-0_acc_score_tol-2.0_err-0.3.png}
            \caption[]%
            {30\% Error Rate}    
            \label{fig:dogfish_svm_03_acc}
        \end{subfigure}
        %\vskip\baselineskip
        %\quad
        \caption[]
        {SVM on Dogfish dataset: test accuracy of each target model of given error rate with classifiers induced by poisoning points obtained from our attack and the KKT attack.} 
        \label{fig:dogfish_svm_acc}
    \end{figure*}  

%     \sisetup{
% output-open-uncertainty = \pm,
% output-close-uncertainty = ,
% uncertainty-separator = {\,}
% }

\begin{table}[!tb]
\centering
\scalebox{0.77}{
\begin{tabular}{ccccc}
\toprule
Dataset & & Target 0 & Target 1 & Target 2 \\ \midrule
\multirow{2}{*}{Adult} & \# of Poisons & 1866 & 2097 & 2163.3 $\pm$ 2.5 \\
& Lower Bound & 1666.7 $\pm$ 2.4 & 1831.4 $\pm$ 5.0 & 1863.0 $\pm$ 9.2 \\ \midrule
 \multirow{2}{*}{Dogfish} & \# of Poisons & 32 & 89 $\pm$ 2.3 & 169 $\pm$ 3.0 \\
  & Lower Bound & 13 & 36 & 67 \\ \bottomrule
\end{tabular}
}
\caption{Optimality of our attack. Top row means number of poisoning points used by our attack. Bottom row means the lower bound computed from Theorem~\ref{theorem:lower_bound} for the induced classifiers. All results are averaged over 4 runs, integer value in the cell means we get exactly same value for 4 runs and others are shown with the average and standard error. For Adult dataset, Target 0 - Target 2 denote target models that have 0\% accuracy on the selected three subpopulations. For Dogfish dataset, Target 0 - Target 2 denotes target classifiers of overall test error of 10\%, 20\% and 30\%. 
}
\label{tab:adult_svm_subpop_lower_bound}
\end{table}



\shortsection{Optimality of Our Attack} In order to check the optimality of our attack, we calculate a lower bound on the number of poisoning points needed to induce the model that is induced by the poisoning points that are found by our attack. We calculate this lower bound on the number of poisons using Theorem~\ref{thm:lowerbounds} (details in Section~\ref{sec:lowerbound}). Note that Theorem \ref{thm:lowerbounds} provides a valid lower bound based on any intermediate model. In order to get a lower bound on the number of poisoning points, we only need to use Theorem \ref{thm:lowerbounds} on the encountered intermediate models and report the best one. We do this by running Algorithm~\ref{algorithm} using the induced model (and not the previous target model) as the target model, terminating when the induced classifier is $0.01$-close to the given target model. We then consider all the intermediate classifiers that the algorithm induced across the iterations. 
%The Adult dataset contains many binary features and hence the search process for the point with maximum loss difference is a (non-convex) mixed integer programming problem. To obtain a valid lower bound, we relax the binary features into real valued features in range $[0,1]$ and then compute the lower bound. 
Our calculated lower bound in Table~\ref{tab:adult_svm_subpop_lower_bound} shows that the gap between the lower bound and the number of used poison points is relatively small. This means our attack is nearly optimal in terms of minimizing the number of poisoning points needed to induce the target classifier.






==> marcos.tex <==
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% \usepackage{algorithmic}
\usepackage{amsthm}
\usepackage{todo}
\usepackage{amsmath,amssymb, mathtools}
\usepackage{multirow}
\usepackage{subfig}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\Regret}{\mathsf{Regret}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\N}{{\mathbb N}}
\newcommand{\cR}{\mathchal{R}}
% \newcommand{\argmax}{\operatorname*{argmax}}


\newcommand{\Snote}[1]{{\color{red} Saeed: #1}}

\newcommand{\MNIST}{{MNIST~1\nobreakdash--7}}

\newcommand{\State}{\STATE}
\newcommand{\While}[1]{\WHILE{#1}}
\newcommand{\EndWhile}[1]{\ENDWHILE{#1}}
  \newcommand{\Return}[1]{\textbf{return} #1}

%\newcommand{\ynote}[1]{{\color{blue} Yuan: #1}}

\theoremstyle{definition} % amsthm only
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{setting}{Setting}

\newcommand{\shortsection}[1]{\subsection{#1}}
\newcommand{\shortsectionnp}[1]{\subsection{#1}}

